Performance Evaluation of OTFS Over Measured V2V Channels at 60 GHz

This paper presents an analysis of the Orthogonal Time Frequency Space (OTFS) modulation scheme when applied to realistic vehicular channel situations. OTFS modulates symbols in delay-Doppler domain, hoping to exploit diversity in both. The penalty for doing this is the requirement of complex interference cancellation equalizers, as this domain incurs a strong amount of intercarrier and intersymbol interference. We conduct this analysis using measured millimeter wave vehicular channels, and we assume typical physical layer settings for a performance analysis. Our results show that there is a challenging trade-off between channel conditions that are easy to equalize and channel conditions that allow OFTS to exploit the two-dimensional diversity. In the first case we observe a good overall performance that is barely enhanced by employing OTFS. In the second case performance gain through OTFS is visible, yet with a bad overall performance.

==> latex-base-files/custom_commands.tex <==
\newcommand{\Expectation}[1]{\mathop{\mathrm{E}}\left\{#1\right\}}
\renewcommand{\vec}{\mathbf}
\newcommand{\mat}{\mathbf}

==> latex-base-files/tikzblocks.tex <==

\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\usetikzlibrary{calc}

\pgfsetlayers{background,main,foreground}
\usetikzlibrary{positioning}
% Define a few styles and constants
\tikzstyle{sensor}=[draw, fill=blue!20, text width=8em,
text centered, minimum height=1.5em, rounded corners]
\tikzstyle{ann} = [above, text width=5em]
\tikzstyle{highLevels} = [sensor, fill=red!20]
\tikzstyle{highLevelsHalf} = [sensor, fill=red!20, text width =3em]
\tikzstyle{highLevels2} = [highLevels, text width=4em]
\def\blockdist{2.3}
\def\edgedist{2.5}
\usetikzlibrary{shapes,arrows,decorations.pathreplacing}
\tikzset{
  radiation/.style={
    {decorate,decoration={expanding waves,angle=90,segment length=4pt}}
  },
  antenna/.pic={
    code={\tikzset{scale=5/10}
      \draw[semithick] (0,0) -- (1,4);% left line
      \draw[semithick] (3,0) -- (2,4);% right line
      \draw[semithick] (0,0) arc (180:0:1.5 and -0.5);
      \node[inner sep=4pt] (circ) at (1.5,5.5) {};
      \draw[semithick] (1.5,5.5) circle(8pt);
      \draw[semithick] (1.5,5.5cm-8pt) -- (1.5,4);
      \draw[semithick] (1.5,4) ellipse (0.5 and 0.166);
      \draw[semithick,radiation,decoration={angle=45}] (1.5cm+8pt,5.5) -- +(0:2);
      \draw[semithick,radiation,decoration={angle=45}] (1.5cm-8pt,5.5) --  +(180:2);
    }
  },
  car/.pic={
    \draw[rounded corners=3pt]
    (0.2,0) rectangle (0.8,1);
    % \draw[rounded corners=1pt]
    % (0.25,0.55) rectangle (0.75,0.75);
    \draw (0.25, 0.7) to [bend left] (0.75, 0.7) -- (0.73, 0.55) to [bend right=15] (0.27, 0.55) -- cycle;
    % \draw[rounded corners=1pt]
    % (0.25,0.1) rectangle (0.75,0.25);
    \draw ( 0.25, 0.13) to [bend right=15] (0.75, 0.13) -- (0.73, 0.23) to [bend left=15] (0.27, 0.23) -- cycle;
    % \path (0.45, 0.3) pic[xscale=.07, yscale=0.05, rotate=0] {antenna};
    \draw (0.2, 0.9) to [bend right] (0.35, 1);
    \draw (0.8, 0.9) to [bend left] (0.65, 1);
    \draw (0.2, 0.1) to [bend left] (0.3, 0);
    \draw (0.8, 0.1) to [bend right] (0.7, 0);
  }
}
